BAPO: Boundary-Aware Policy Optimization for Reliable Agentic Search

RL-based agentic search enables LLMs to solve complex questions via dynamic planning and external search. While this approach significantly enhances accuracy with agent policies optimized via large-scale reinforcement learning, we identify a critical gap in reliability: these agents fail to recognize their reasoning boundaries and rarely admit ``I DON'T KNOW'' (IDK) even when evidence is insufficient or reasoning reaches its limit. The lack of reliability often leads to plausible but unreliable answers, introducing significant risks in many real-world scenarios. To this end, we propose Boundary-Aware Policy Optimization (BAPO), a novel RL framework designed to cultivate reliable boundary awareness without compromising accuracy. BAPO introduces two key components: (i) a group-based boundary-aware reward that encourages an IDK response only when the reasoning reaches its limit, and (ii) an adaptive reward modulator that strategically suspends this reward during early exploration, preventing the model from exploiting IDK as a shortcut. Extensive experiments on four benchmarks demonstrate that BAPO substantially enhances the overall reliability of agentic search.

==> backup-intro.tex <==
% Recently released RL-based agentic search models, such as Search-R1 and ReSearch~\cite{search-r1, research}, have exhibited advanced performance on search task based on their dynamic retrieval strategies during reasoning process.
Recently released RL-based agentic search models, such as Search-R1~\cite{search-r1} and ReSearch~\cite{research}, extend reinforcement learning (RL) for agentic reasoning to enable LLMs to autonomously generate multiple search queries during step-by-step reasoning with real-time retrieval. 
As these cutting-edge agentic models take on increasingly complex questions where the verification of their search results is challenging for human, ensuring the reliability of search results is critical to avoid misleading users.
Therefore, when the model cannot reach a concrete final answer due to its limited reasoning ability or a lack of relevant information in retrieved text, we expect it to admit \textit{``I DON'T KNOW''}(\textit{IDK}) to prevent fabricated answer. Furthermore, showing the failed reasoning trajectories helps users adjust their questions or turn to more professional sources for answers.
% 作为一种高自主性的agentic搜索范式，这种系统为用户能解决更多更复杂的问题之时，应更加注意搜索的精确性，以避免错误的搜索结果对用户的误导。when a question cannot lead to a concrete final answer due to insufficient model reasoning ability or a lack of relevant knowledge in network or knowledge base，我们希望search models具备可以承认不知道来避免给出误导性结果，保留的搜索轨迹可以帮助用户去调整他的问题或从其他更专业信息源寻找回答。
%作为一种高自主性的 Agentic 搜索范式，此类系统虽然能协助用户解决更复杂的难题，但也因此必须更加注重搜索的精确性，以防止错误结果误导用户。
%当由于模型推理能力不足，或网络/知识库中缺乏相关知识而导致无法得出确切答案时，我们希望搜索模型具备‘拒答’的能力，从而避免产生误导性结果。失败的搜索轨迹也可以帮助用户调整问题，或转向更专业的信息源寻求答案。


% whether an user's search can yield an answer often stems from various factors. These include insufficient model reasoning ability, unsolvable user question, or a lack of relevant knowledge in the network or knowledge base~\cite{rejectionIR, reliablemath}. However, when the reasoning process cannot lead to a concrete final answer, these search systems tend to give an uncertain answer rather than admitting the unavailability of a final answer.
% 从boundary角度来写
% Previous work 将这类情况归结为boundary where the problem is 超出了模型可以回答的boudnary. 某某提出knowledge boundary的概念用以解释模型遇到超出自己参数化知识能力的问题，Qiu提出capability boundary用以解释open-source LRM models推理过程中高难度的问题超出模型的推理能力overlook the relationship between questions and LRMs' capability boundaries. 对于agentic search models，由于采用动态的检索信息和推理相结合的方式，模型需要根据检索的内容来明确自己的Reasoning capability表示模型根据自己的推理轨迹才能明确自己对于问题是否可答。
% To improve model's reliability, previous work employs a reliable prompting method to hint models answer \textit{I DON'T KNOW} if they can't give a confident answer of the question~\cite{rejectionIR, reliablemath}. 
\input{tables/table1}

Prior research attributes the ability to admit \textit{IDK} to LLM's \textbf{awareness of its ``boundary''} where problems exceed the it's answerable scope. ~\citet{knowledgeboundarylargelanguageli2025} treat knowledge boundary as model's parameterized knowledge, while ~\citet{ontheselfawareness_2025} introduce the concept of capability boundary to explain the struggling of large reasoning models when facing complex tasks that exceeds their reasoning capability.
In contrast, the boundary of agentic search models is not solely determined by their predefined reasoning capability, but also significantly related to the dynamically retrieved information. 
Therefore, we define its \textbf{reasoning boundary} as the reachability of a concrete final answer based on the information gathered along the model's reasoning trajectory. Improving the model's awareness of its reasoning boundary is key to enhance the reliability of agentic search models.

% Table1的结论：However, our preliminary study reveals that even equipped with a reliable prompt indicating model to reject answer and output \tetxit{``I DON'T KNOW'' (IDK)} when it can't a concrete final answer at the end of the reasoning, the RL trained model still tend to give an unreliable answer rather than admitting \tetxit{IDK}, wheres instruct models before agentic RL 却可以有效拒绝回答。
% % 模型的这种行为在RL训练之前是

% they can't 
% when a question cannot lead to a concrete final answer due to insufficient model reasoning ability or a lack of relevant knowledge in network or knowledge base, these models still tend to give an unreliable answer rather than admitting the unavailability of a final answer.
As a widely adopted method for eliciting LLM's awareness of its boundaries, reliable prompting is 
% used to elicit the LLM's awareness of its boundaries, encouraging it to refuse to answer when appropriate~\cite{rejectionIR,reliablemath}. Specifically, this is 
implemented by appending the following instruction to the end of the prompt~\cite{rejectionIR,reliablemath}:
\begin{tcolorbox}[colback=gray!10, colframe=gray!60, title=Reliable Prompt]
\texttt{If you can't solve this question by the reasoning process, you should output \textbackslash boxed\{I DON'T KNOW\}}
\end{tcolorbox}
However, our preliminary experiments, as presented in Table~\ref{tab:table1}, reveal a critical finding: As the accuracy increases after RL training, the effectiveness of reliable prompting in activating their boundary awareness diminishes. The reason why models after RL struggle to exhibit reliability lies in the misalignment between existing RL algorithms’ reward functions and human expectations for model reliability.

%基于RL的正确性奖励和现实中用户对reliability的要求这一mismatch这一点观察，我们提出了一个算法，基于GRPO，一组中的答案的表现，动态决定是否奖励模型去承认IDK，我们的算法基于一个基本假设————如果模型的多次采样的回答都难以解决一个问题，那么这个问题超出了模型的推理边界，此时应该鼓励模型去回答IDK，惩罚没有拒绝回答的轨迹，反之，如果一组回答中出现正确答案，那么可以认为这个问题处于模型推理范围内，此时应该奖励正确的轨迹，惩罚错误的和IDK。通过在恰当的时候鼓励IDK，我们希望这样的奖励能让模型build出self-awareness of its reasoning boundary.
%然而，一个关键的挑战在于如何动态平衡模型的能力增长和边界意识。新的奖励给模型学习提供了一个shortcut，让模型直接承认IDK而不去尝试解决难的问题，带来解决问题能力的过早停滞。为此，我们也提出了一种动态的奖励机制来实现模型解决问题能力和边界意识的balance，通过在早期探索阶段，和在高探索价值的问题上deactivate 奖励IDK轨迹，使得模型在边界意识和解决问题能力上达到一个balance。
To address the mismatch, we propose \textbf{Reasoning-Boundary Aware Policy Optimization (RAPO)}, a new RL methods building upon GRPO~\cite{deepseekmath_shao_2024}. Based on the commonly used correct and format reward~\cite{research}. RAPO introduces a new \textbf{Reasoning-Boundary Aware Reward} to dynamically decide whether to reward the model for admitting \textit{IDK} based on the performance of a group of rollouts. It is grounded in a fundamental assumption: if multiple rollouts from the model struggle to solve a problem, it indicates that the problem exceeds the model's reasoning boundary. In such cases, the model should be encouraged to answer \textit{IDK}, and trajectories that gives a wrong answer should be penalized. Conversely, if at least one correct trajectory appears within a group of rollouts, the problem is considered within the model's reasoning boundary, and correct trajectories should be rewarded while incorrect ones and \textit{IDK} responses are penalized. 
By appropriately encourage and penalize \textit{IDK} responses, the model develops the self-awareness of its reasoning boundary.

However, a key challenge lies in dynamically balancing the model's problem-solving capability and boundary awareness. The new
Reasoning-Boundary Aware Reward introduces a potential shortcut for the model to simply admit \textit{IDK} without attempting to solve difficult problems, leading to premature stagnation in problem-solving ability. Therefore, we further propose a dynamic reward mechanism to deactivate the reward for \textit{IDK} trajectories during the early exploration training stage and on high-exploration-value questions, thereby achieving a balance between the model's problem-solving capability and boundary awareness.

Our contributions are summarized as follows:
\begin{itemize}
\item We identify the limitations of existing RL algorithms that solely reward correctness, which compromises model reliability. To address this, we propose RAPO, a novel RL algorithm that dynamically rewards \textit{IDK} responses to cultivate the model's self-awareness of its reasoning boundaries.
\item Our proposed adaptive reward mechanism achieves a balance between model's boundary awareness and problem-solving capability.
\item Extensive experiments on challenging benchmarks demonstrate that RAPO effectively enhances search reliability while preserving the model's ability to solve complex problems.
\end{itemize}
%我们的贡献可以总结为以下几点：
%1.我们揭示了现有RL算法正确性的奖励
%2.提出了Reward
%3


%Changllge
% To improve model reliability, reliable prompting has been 证实是一个简单有效的方法，however, when we apply it int
% Therefore, 我们用the reasoning boundary to define the 可得性 of a final answer that can be supported by the information obtained within the interleved reasoning-retrival trajectory.
% In contrast, the boundary of agentic search models is not only depends on model's predefined reasoning ability, but also relevant to the retrived information during reasoning. therefore, 我们定义了模型的reasoning boundaries as model已有的reasoning trajetory中的得到的信息能得出的支撑的结论范围。

% instead, the model assesses its ability to answer a question only after executing its reasoning trajectory and engaging with retrieved content. This means their effective capability boundary is determined dynamically during the reasoning process itself.

% When adopting reliable prompting to Qwen2.5-7B-Instruct, the model achieves higher precision while at the minor cost of lower accuracy when compared to the orginal prompt. After the model's training on GRPO, the reliable prompt can't bring enough boost to the reliability.



==> tables/table1.tex <==
\begin{table}[t]
% \small
    \centering
    % \small
    \begin{tabular}{llll}
    \toprule
    \textbf{Method} & \textbf{EM} & \textbf{LJE} & \textbf{RR} \\
    \midrule
    \multicolumn{4}{l}{\cellcolor[gray]{0.85}\textit{Instruct Model (Before RL)}} \\
    \quad \makecell{\textbf{Accuracy}\\ \textbf{Precision}}    & 37.0 & 57.0 & - \\
    \multicolumn{4}{l}{\cellcolor[gray]{0.93}\textit{+reliable prompt}} \\
    \quad \textbf{Accuracy}    & 36.0\textsubscript{ \textcolor{ForestGreen}{($\downarrow$1.0)}} & 55.5\textsubscript{ \textcolor{ForestGreen}{($\downarrow$1.5)}} & \multirow{2}{*}{17\%} \\ 
    \quad \textbf{Precision}   & 43.6\textsubscript{ \textcolor{red}{($\uparrow$6.6)}} & 67.2\textsubscript{ \textcolor{red}{($\uparrow$10.2)}} & \\
    \midrule
    \multicolumn{4}{l}{\cellcolor[gray]{0.85}\textit{Agentic Reasoning Model (After RL)}} \\
    \quad \makecell{\textbf{Accuracy}\\ \textbf{Precision}}  & 46.0 & 63.5 & - \\
    \multicolumn{4}{l}{\cellcolor[gray]{0.93}\textit{+reliable prompt}} \\
    \quad \textbf{Accuracy}  & 46.5\textsubscript{ \textcolor{red}{($\uparrow$0.5)}} & 63.0\textsubscript{ \textcolor{ForestGreen}{($\downarrow$0.5)}} & \multirow{2}{*}{3.5\%} \\ 
    \quad \textbf{Precision}   & 48.1\textsubscript{ \textcolor{red}{($\uparrow$2.1)}} & 65.2\textsubscript{ \textcolor{red}{($\uparrow$1.7)}} & \\
    % \midrule
    % \textbf{Average Acc.}  &  &  \\
    \bottomrule
    \end{tabular}
    \caption{Performance of F1, Exact Match (EM), Rejection Rate (RR) and LLM-as-a-Judge Equal (LJE) results on multi-hop QA benchmark HotpotQA. Here we choose GRPO as RL algorithm. \\\textcolor{blue}{[TODO: Change it into a figure (bar chart)]}}
    % \vspace{-3ex}
    \label{tab:table1}
\end{table}
